Experiences of Censorship on TikTok Across Marginalised Identities

TikTok has seen exponential growth as a platform, fuelled by the success of its proprietary recommender algorithm which serves tailored content to every user - though not without controversy. Users complain of their content being unfairly suppressed by ''the algorithm'', particularly users with marginalised identities such as LGBTQ+ users. Together with content removal, this suppression acts to censor what is shared on the platform. Journalists have revealed biases in automatic censorship, as well as human moderation. We investigate experiences of censorship on TikTok, across users marginalised by their gender, LGBTQ+ identity, disability or ethnicity. We survey 627 UK-based TikTok users and find that marginalised users often feel they are subject to censorship for content that does not violate community guidelines. We highlight many avenues for future research into censorship on TikTok, with a focus on users' folk theories, which greatly shape their experiences of the platform.

==> ethics.tex <==
\newpage
%\subsection{Ethical Statement}

%All data was from pseudo-anonymised accounts on Prolific,  minimising the risk of loss of privacy should our data be leaked. Data stored on Qualtrics (which meets the high security standards) or held and analysed on secure laptops. 


\subsection{Paper Checklist to be included in your paper}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes, we gather data using best practice from existing social media research and framed our demographic questions in line with the UK Census to avoid offence. Our descriptive analysis captures self-reported behaviour, and does not make a value judgement or try to predict/ profile users.}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes, we provide a succinct summary of the paper in the abstract and justify our interest in the topic and the scope of the paper in the Introduction.}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes, as we mention in Procedure and Measurements this is an exploratory analysis, and we do not attempt to prove any hypotheses but rather report current behaviour.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, see Limitations.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, see Limitations.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes, see limitations.}
      \item Did you discuss any potential misuse of your work?
    \answerYes{Yes, see limitations.}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes, protocol for the survey is publicly available (see Supplementary Material) but we do not release the data to protect privacy.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes.}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerNA{NA}
  \item Have you provided justifications for all theoretical results?
    \answerNA{NA}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{NA}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerNA{NA}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerNA{NA}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerNA{NA}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{NA}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{NA}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{NA}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{NA}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerNA{NA}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerNA{NA}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{NA}
  \item Did you mention the license of the assets?
    \answerNA{NA}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerNA{NA}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{NA}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{NA}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR (see \citet{fair})?
\answerNA{NA}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \citet{gebru2021datasheets})? 
\answerNA{NA}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerYes{Yes, see Supplementary Material (Consent Page currently redacted to protect anonymity)}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerYes{Yes, see Supplementary Material (Consent Page currently redacted to protect anonymity)}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{Yes, see Methodology.}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerYes{Yes, see Methodology.}
\end{enumerate}

\end{enumerate}



==> format.tex <==
\subsection{Overlength Papers}
If your paper is too long and you resort to formatting tricks to make it fit, it is quite likely that it will be returned to you. The best way to retain readability if the paper is overlength is to cut text, figures, or tables. There are a few acceptable ways to reduce paper size that don't affect readability. First, turn on \textbackslash frenchspacing, which will reduce the space after periods. Next, move all your figures and tables to the top of the page. Consider removing less important portions of a figure. If you use \textbackslash centering instead of \textbackslash begin\{center\} in your figure environment, you can also buy some space. For mathematical environments, you may reduce fontsize {\bf but not below 6.5 point}.


Commands that alter page layout are forbidden. These include \textbackslash columnsep,  \textbackslash float, \textbackslash topmargin, \textbackslash topskip, \textbackslash textheight, \textbackslash textwidth, \textbackslash oddsidemargin, and \textbackslash evensizemargin (this list is not exhaustive). If you alter page layout, you will be required to pay the page fee. Other commands that are questionable and may cause your paper to be rejected include \textbackslash parindent, and \textbackslash parskip. Commands that alter the space between sections are forbidden. The title sec package is not allowed. Regardless of the above, if your paper is obviously ``squeezed" it is not going to to be accepted. Options for reducing the length of a paper include reducing the size of your graphics, cutting text, or paying the extra page charge (if it is offered).


\subsubsection{Section Headings.}
Sections should be arranged and headed as follows:
\begin{enumerate}
\item Main content sections
\item Appendices (optional)
\item Ethical statement (optional, unnumbered)
\item Acknowledgements (optional, unnumbered)
\item References (unnumbered)
\end{enumerate}



\subsubsection{Ethical statement.}
You can write a statement about the potential ethical impact of your work, including its broad societal implications, both positive and negative. If included, such statement must be written in an unnumbered section titled \emph{Ethical statement}.

\subsubsection{References.}
The references section should be labeled ``References" and must appear at the very end of the paper (don't end the paper with references, and then put a figure by itself on the last page). A sample list of references is given later on in these instructions. Please use a consistent format for references. Poorly prepared or sloppy references reflect badly on the quality of your paper and your research. Please prepare complete and accurate citations.

\subsection{Illustrations and  Figures}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{figure1} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{Using the trim and clip commands produces fragile layers that can result in disasters (like this one from an actual paper) when the color space is corrected or the PDF combined with others for the final proceedings. Crop your figures properly in a graphics program -- not in LaTeX}.
\label{fig1}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{figure2} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Adjusting the bounding box instead of actually removing the unwanted data resulted multiple layers in this paper. It also needlessly increased the PDF size. In this case, the size of the unwanted layer doubled the paper's size, and produced the following surprising results in final production. Crop your figures properly in a graphics program. Don't just alter the bounding box.}
\label{fig2}
\end{figure*}

% Using the \centering command instead of \begin{center} ... \end{center} will save space
% Positioning your figure at the top of the page will save space and make the paper more readable
% Using 0.95\columnwidth in conjunction with the


Your paper must compile in PDF\LaTeX{}. Consequently, all your figures must be .jpg, .png, or .pdf. You may not use the .gif (the resolution is too low), .ps, or .eps file format for your figures.

Figures, drawings, tables, and photographs should be placed throughout the paper on the page (or the subsequent page) where they are first discussed. Do not group them together at the end of the paper. If placed at the top of the paper, illustrations may run across both columns. Figures must not invade the top, bottom, or side margin areas. Figures must be inserted using the \textbackslash usepackage\{graphicx\}. Number figures sequentially, for example, figure 1, and so on. Do not use minipage to group figures.

If you normally create your figures using pgfplots, please create the figures first, and then import them as pdfs with proper bounding boxes, as the bounding and trim boxes created by pfgplots are fragile and not valid.

When you include your figures, you must crop them \textbf{outside} of \LaTeX{}. The command \textbackslash includegraphics*[clip=true, viewport 0 0 10 10]{...} might result in a PDF that looks great, but the image is \textbf{not really cropped.} The full image can reappear (and obscure whatever it is overlapping) when page numbers are applied or color space is standardized. Figures \ref{fig1}, and \ref{fig2} display some unwanted results that often occur.

If your paper includes illustrations that are not compatible with PDF\TeX{} (such as .eps or .ps documents), you will need to convert them. The epstopdf package will usually work for eps files. You will need to convert your ps files to PDF in either case.

\subsubsection {Figure Captions.}The illustration number and caption must appear \textit{under} the illustration. Labels and other text with the actual illustration must be at least nine-point type. However, the font and size of figure captions must be 10 point roman. Do not make them smaller, bold, or italic. (Individual words may be italicized if the context requires differentiation.)

\subsection{Tables}

Tables should be presented in 10 point roman type. If necessary, they may be altered to 9 point type. You may not use any commands that further reduce point size below nine points. Tables that do not fit in a single column must be placed across double columns. If your table won't fit within the margins even when spanning both columns, you must split it. Do not use minipage to group tables.

\subsubsection {Table Captions.} The number and caption for your table must appear \textit{under} (not above) the table.  Additionally, the font and size of table captions must be 10 point roman and must be placed beneath the figure. Do not make them smaller, bold, or italic. (Individual words may be italicized if the context requires differentiation.)

\subsubsection{Using Color.}
Use of color is restricted to figures only. It must be WACG 2.0 compliant. (That is, the contrast ratio must be greater than 4.5:1 no matter the font size.) It must be CMYK, NOT RGB. It may never be used for any portion of the text of your paper. The archival version of your paper will be printed in black and white and grayscale. The web version must be readable by persons with disabilities. Consequently, because conversion to grayscale can cause undesirable effects (red changes to black, yellow can disappear, and so forth), we strongly suggest you avoid placing color figures in your document. If you do include color figures, you must (1) use the CMYK (not RGB) colorspace and (2) be mindful of readers who may happen to have trouble distinguishing colors. Your paper must be decipherable without using color for distinction.

\subsubsection{Resizing Graphics.}
Resize your graphics \textbf{before} you include them with LaTeX. You may \textbf{not} use trim or clip options as part of your \textbackslash includegraphics command. Resize the media box of your PDF using a graphics program instead.


\subsection{References}
The AAAI style includes a set of definitions for use in formatting references with BibTeX. These definitions make the bibliography style fairly close to the ones  specified in the Reference Examples appendix below. To use these definitions, you also need the BibTeX style file ``aaai22.bst," available in the AAAI Author Kit on the AAAI web site. Then, at the end of your paper but before \textbackslash end{document}, you need to put the following lines:

\begin{quote}
\begin{small}
\textbackslash bibliography\{bibfile1,bibfile2,...\}
\end{small}
\end{quote}

Please note that the aaai22.sty class already sets the bibliographystyle for you, so you do not have to place any \textbackslash bibliographystyle command in the document yourselves. The aaai22.sty file is incompatible with the hyperref and navigator packages. If you use either, your references will be garbled and your paper will be returned to you.

References may be the same size as surrounding text. However, in this section (only), you may reduce the size to \textbackslash small if your paper exceeds the allowable number of pages. Making it any smaller than 9 point with 10 point linespacing, however, is not allowed. A more precise and exact method of reducing the size of your references minimally is by means of the following command: \begin{quote}
\textbackslash fontsize\{9.8pt\}\{10.8pt\}
\textbackslash selectfont\end{quote}

\noindent You must reduce the size equally for both font size and line spacing, and may not reduce the size beyond \{9.0pt\}\{10.0pt\}.

The list of files in the \textbackslash bibliography command should be the names of your BibTeX source files (that is, the .bib files referenced in your paper).

The following commands are available for your use in citing references:
\begin{quote}
{\em \textbackslash cite:} Cites the given reference(s) with a full citation. This appears as ``(Author Year)'' for one reference, or ``(Author Year; Author Year)'' for multiple references.\smallskip\\
{\em \textbackslash shortcite:} Cites the given reference(s) with just the year. This appears as ``(Year)'' for one reference, or ``(Year; Year)'' for multiple references.\smallskip\\
{\em \textbackslash citeauthor:} Cites the given reference(s) with just the author name(s) and no parentheses.\smallskip\\
{\em \textbackslash citeyear:} Cites the given reference(s) with just the date(s) and no parentheses.
\end{quote}
You may also use any of the \emph{natbib} citation commands.


\appendix
\section{Reference Examples}
\label{sec:reference_examples}

\nobibliography*
Formatted bibliographies should look like the following examples. You should use BibTeX to generate the references. Missing fields are unacceptable when compiling references, and usually indicate that you are using the wrong type of entry (BibTeX class).

\paragraph{Book with multiple authors~\nocite{em:86}} Use the \texttt{@book} class.\\[.2em]
\bibentry{em:86}.

\paragraph{Journal and magazine articles~\nocite{r:80, hcr:83}} Use the \texttt{@article} class.\\[.2em]
\bibentry{r:80}.\\[.2em]
\bibentry{hcr:83}.

\paragraph{Proceedings paper published by a society, press or publisher~\nocite{c:83, c:84}} Use the \texttt{@inproceedings} class. You may abbreviate the \emph{booktitle} field, but make sure that the conference edition is clear.\\[.2em]
\bibentry{c:84}.\\[.2em]
\bibentry{c:83}.

\paragraph{University technical report~\nocite{r:86}} Use the \texttt{@techreport} class.\\[.2em]
\bibentry{r:86}.

\paragraph{Dissertation or thesis~\nocite{c:79}} Use the \texttt{@phdthesis} class.\\[.2em]
\bibentry{c:79}.

\paragraph{Forthcoming publication~\nocite{c:21}} Use the \texttt{@misc} class with a \texttt{note="Forthcoming"} annotation.
\begin{quote}
\begin{footnotesize}
\begin{verbatim}
@misc(key,
  [...]
  note="Forthcoming",
)
\end{verbatim}
\end{footnotesize}
\end{quote}
\bibentry{c:21}.

\paragraph{ArXiv paper~\nocite{c:22}} Fetch the BibTeX entry from the "Export Bibtex Citation" link in the arXiv website. Notice it uses the \texttt{@misc} class instead of the \texttt{@article} one, and that it includes the \texttt{eprint} and \texttt{archivePrefix} keys.
\begin{quote}
\begin{footnotesize}
\begin{verbatim}
@misc(key,
  [...]
  eprint="xxxx.yyyy",
  archivePrefix="arXiv",
)
\end{verbatim}
\end{footnotesize}
\end{quote}
\bibentry{c:22}.

\paragraph{Website or online resource~\nocite{c:23}} Use the \texttt{@misc} class. Add the url in the \texttt{howpublished} field and the date of access in the \texttt{note} field:
\begin{quote}
\begin{footnotesize}
\begin{verbatim}
@misc(key,
  [...]
  howpublished="\url{http://...}",
  note="Accessed: YYYY-mm-dd",
)
\end{verbatim}
\end{footnotesize}
\end{quote}
\bibentry{c:23}.

\vspace{.2em}
For the most up to date version of the AAAI reference style, please consult the \textit{AI Magazine} Author Guidelines at \url{https://aaai.org/ojs/index.php/aimagazine/about/submissions#authorGuidelines}

% Use \bibliography{yourbibfile} instead or the References section will not appear in your paper
\nobibliography{aaai22}

==> notes.tex <==
GENERAL NOTES
Higher counts of suppression than removal even though similar number respondents. So those who suspected suppression suspected it over more topics. 

GENDER NOTES

Men more likely to post political content and unsurprisingly more likely to say it is removed, but similar reports of suppression.  Similar levels of agreement for algorithmic suppression (neither agree or disagree) and community guidelines (slight disagree)

Men more likely to post content some may find offensive, unsurprisingly more likely to report it being removed, but similar reports of suppression. Similar levels of agreement for algorithmic suppression (slightly agree). Nonbinary neither agree or disagree for community guidelines, men and women agree. 

Women less likely to post nonerotic sex content but report similar rates of censorship. Women agree is algo censored, men and nonbinary neither agree disagree. All slightly disagree goes against comm. guidelines 

Men more likely to post erotic content. Nonbinary never. Same rate removal across male female. Men four counts suppression, women nonbinary none. All agree gets algo censored, women and nonb most strongly. All agree goes against comm guidelines. 

Men post more covid content but similar reports of suppression compared to women. Nonb most strongly disagree is algo censored, goes against comm guidelines. 

Enby more likely to crit dom group, similar male and female. Same count of suppression and censorship across genders (low levels). Women and enby slightly more strongly agree is algo censored. neither agree disagree against com guielines for all. 

Men SJ content more than women, enby most. Men removed, others none. Similar counts suppression men women. None enby. Men dont know algo censored, women and enby agree is censored. All disagree goes against comm guidelines, enby most strongly. 

Enby v likely to post about minority experience (50\%), men and women similar. Wmoen 2 removals, others none. Women most suppression (4), others 2. Men dont know algo censor, women agree, nonbinary agree most. All disagree against com guidelines, nonbinary strongly. 

Men post most hate speech (5\%!), nonbinary none, women a little. 1 removal, male. 2 suppression for male and female. All agree algo censored, similar levels. All agree against comm guidelines (but the men post anyway!). 

Similar level curse words use. Similar level censorship. enby Not clear if algo censored, men women slightly agree, all slightly slightly disagree against com guidelines. 

1 in 10 men and enby use self slurs, more than women. More counts men use slurs but similar counts removal and suppression. None for enby. All agree gets algo censored, men and enby most strongly (even tho enbies not report any removal or suppresion!). All slightly agree against com guidelines, similar levels. 

Men most likely to post non shock violence, report more removal and suppress. men women slightly agree algo censored, enby neither. men women not sure against comm guidelines, enby slight disagree. 

Men post more violent shock content. Enbys none. But women report more removal, men more suppression. All agree algo censored, women most. All agree against comm guidelines. 

Interestingly, men place more blame for algo/comguide mismatches on human moderators. 

TRANS STATUS NOTES

ONLY 6 TRANS, hard to find quan differences. 
No trans report any content removal but some reports of suppression. 

Similar levels political content posting, all removal and suppression from non-trans, trans more agree algo censored, nontrans neither ag or disag, both disagree goes against com guidelines but nontrans more so. 

similar levels some find offensive. all removal and suppress nontrans. both agree censored, trans more so. both slightly agree against com guideines, nontrans more so. 

Trans never sex non erotic - though one reported suppression of this. nontrans slightly agree censored, trans not sure. nontrans not sure if goes against com, nontrans slightly disagree.

trans never sex erotic but again one report suppression. nontrans agree algo censored more than trans. both agree against com guideline, trans more strongly. 

one trans report covid content, same percentage as nontrans (15\% ). trans disagree algo censored, nontrans neither. both disagree against com guidelines, nontrans more so. 

no trans post crit dom group. 8\% non trans. only nontrans report suppression.  trans disagree algo censored, nontrans agree. trans agree against com guidelines, nontrans neither. 

1 trans posted sj content, similar percentage nontrans (17\%). only nontrans report suppression. trans not sure algo censored, nontrans slightly agree. trans agree against comm guidelines, nontrans disagree. 

unsurprinsgly, trans more likely to post about minority identity experience. 1 reported suppression, so higher rate of suppression amongst trans. both slightly agree algo censored. both slightly disagree against com guidelines.

no trans post hatespeech. suppression of hate speech not even that high.  both agree algo censored but trans less strngly. both agree against comm guidelines, trans more so. 

non trans post cursewords much more (hard to tell with so few trans tho). trans disagree algo censor, nontrans agree. trans slightly slight agree against com guidelines, nontrans slightly slight disagree. 

no trans self ref slur. agree algo censored but trans a lot more. agree against com guidelines, trans more so. 

trans no violence onshock content. agree algo censored, trans more strongly. trans think against com guidelines, nontrans not sure. 

trans no violence shock content. both agree algo censored, both agree against com guidelines. 

trans agree algo trained stricted guidelines most strongly, then human mods have own opinion, then user report. nontrans most strong agree human report, then mod opions, then mistakes. 

SEXUALITY NOTES

NOTE ACE OFTEN MORE DISAGREE BUT THIS IS NOT DATA QUALITY ISSUE, NO SINGLE ACE PARTICIPANT CONSISTENTLY GIVES LOW ANSWER FOR EXAMPLE

LGB+ participants more likely than straight to post political content (tho obvs fewer numbers). Despite this, straight and bi report exact same count of removal and suppression so rate is MUCH higher for bisexuals. Despite this, bi and straight not sure if subject to algo censorship, only slightly above 3. Ace disagree, Gay agree. All disagree against community guidelines.

Straight and bi post similar levels "some may find offensive" but straight twice as likely to report this being removed, suggesting what bi and straight consider some may find offensive, is more true for straights? same likelihood suppression. all agree algo censored, less strongly agree against com guidelines (except ace who disagree). 

straight similar likely to bi post sex nonerotic, more likely to post frequently. more straights post but same count of removal for straight and bi (1 each). straight think suppressed, bi not. 1 gay post and they think suppressed. bi, gay, ace believe algo censored more strongly than straight. all disagree against com guidelines, but bisexual only v weakly.

straight more likely to post erotic, only who reports removal. 1 gay reports suppression despite no gay report posting. all agree algo censored ace most strongly. all agree against community guidelines, straight least strongly. 

bis face slightly more censorship for covid. no one sure if algo censored, except ace who disagree. all disagree against com guidelines.

LGB+ more likely to post crit dom group. 
similar likely remove and suppress across straight and bi, none for gay. bi straight ace agree algo censored, gay not sure. not sure if against com guidelines, ace disagree. 

LGB+ more likely to post SJ content (around 30\% compared to straight 15\%). Only 1 straight, 1 gay report removal. 7 straight report suppression, 2 bi - 63 straights post, 26 bi. bi and gay agree algo censored, straight and ace weakly agree. all disagree against comm guidelies, ace especially so. 

unsurprisingly, lGB+ much more likely to post minority identity experience (over 30\%). similar count of bi and straight posting but only bi report removal (n=2). high numbers bisexual believe suppressed (6 which would be $1/4$ everyone who posted). all agree subject to algo censorship,LGB+ more strongly than straight. all disagree against community guidelines, ace most strongly. 


gay and ace most likely to report hate speech but hard to interpret this given low ace count. only straight report censorship. all agree algo censored, ace weakest agree. all agree against community guidelines, ace most strongly, straight weakest. 

bisexuals most likely to report posting curse words. rate of removal higher for bis than straights. suppression about same. all weakly agree algo censored except ace who not sure. all disagree against comm guidelines except gay not sure. 

gay most likely to use slur (maybe unsurprising given example is dyke). same count of bi and straight report removal (1) so 3 times higher likely for bi. same level suppression. all agree algo censored, bisexual most strongly so. weakly agree against comm guidelines. 

non shock violence post similar levels, except ace none. 2 bi, 2 straight report removal so more likely for bi. similar levels suppression. all agree algo censored except ace who disagree. gay straight not sure if against comm guidelines, bi weakly disagree, ace disagree. 

straight most likely violent shock content. bi overly censored for this compared to straight. all agree algo censored, bi most strongly. all agree against com guidelines, bi most strongly. 

across sexualities, most agree others reporting is why mismatch. no other obvious patterns. 

DISABILITY NOTES


similar rates posting political content, but dis seems overly likely to be censored. neither sure if algo censored, both disagree against comm guidelines. 

dis post more some may find offensive. similar rates removal, suppression. agree algo censore, agree against com guidelines but nondis less strong. 

similar rates non erotic sex posting, similar rates censorship (non censored dis but also low posting count). both agree algo censored but nondis less strong. dis not sure if against com guidelines, nondis disagree. 


similar rates sex content. no dis report censor but also low posting counts. agree algo censored, dis most strongly. both agree against com guidelines, dis more strongly. 

nondis post slightly more covid, but only disabled had content removed which is v high rate as so few posted. suspected suppression likelihood in line with posting. nondis slightly disagree algo censored, dis not sure. both disagree against com guidelines. 

dis slightly more likely to post crit dom group. censorship counts in line with posting counts. agree algo censored, dis more strongly. neither sure if against com guidelines. 

similar rates SJ post, censorship in line with these counts. agree algo censored, dis more strongly. disagree against comm guidelines. 

dis lots more likely to post about minority experience. (25\% vs 10\%). based on counts, dis more likely to have removed or be suppressed. agree algo censored, dis more so, disagree against com guidelines. 

similar low levels hate speech. only nondis censored. both agree algo censor, nondis more strongly. both agree against comm guidelines, dis more strong. 

dis curse more (50\%). similar levels censorship, maybe dis suspect more suppression. agree algo censored, dis more so. nondis disagree against com guidelines, dis weakly agree. 

dis more likely use slur. only nondis censored. agree algo censored, dis more strongly. weakly agree against com guidelines, dis more strongly. 

nondis more non shock violence. dis not overly censored. agree algo censored, not sure if against com guidelines. 

similar level violence, accounts for 2 dis posting violence, both reported removed. agree algo censored and against com guidelines. 

v similar opinions about mismatches.

ETHNICITY NOTES

white least likely to post political content. black most likely, almost 50\%. higher rates of suppression for mixed and asian than would expect. nonwhite weakly agree algo censored, white not sure. all disagree against comm guidelines, white most so. 

black most likely post some find offensive. 
whites maybe report slightly higher than expected removal, asian definitely do. removal and suppression reports similar. all agree algo censored, mixed most. all agree against com guidelines, mixed most. 

black post most nonerotic sex, similar rates censorship across groups. all agree algo censored, differences whether believe against com guidelines (black not sure and they post most, everone else disagree). 

black most likely post erotic, but no removal. all agree algo censored, mixed most strongly (only 1 mixed posted and 1 say suppressed). all agree against com guidelines, mixed most strongy. 

black most likely post covid. much higher suspected rate suppression (3 counts to white 4 when so many more white0. variation across ethnicities if algo censored, white disagree mixed agree. all disagree against com guidelines, white most strong. 

black most crit dom group, mixed asian only slightly more than white. white black similar counts censorship suggesting blck would be over censored (but stil n=1 or 2). asian not sure algo censored, whit slight agree, mixed and black more agree. white not sure against com guidelines, mixed and black agree, asian week disagree. 

nonwhite post more SJ content, black most. only 1 report sj content removed, asian (plus 1 "another"). nonwhite overly likely to think suppressed. all agree algo censored except black, not sure. all disagree against com guidelines. 

unsurprisingly, white post least minority identity experience content. hard to interpret removal/suppression of white as likely related to another form of marginalisation. all agree algo censored, mixed most so. all disagree against com guidelines, asian most so. 

mixed  most likely hate speech, tho n=2. similar levels censorship across groups. all agree algo censored (except to "another"). all agree against com guidelines, white most so. 

white report most curse words. nonwhite maybe censored more than expected (worth looking into whether curse words used by certain communities are penalised more). all agree algo censored, mixed most so ("another disagree"). black not sure against com guidelines, everyone else disagree (another agree). 

black and mixed use most self referential slur. censorship as expected.  all agree algo cnesored, mixed most. asian not sure against com guidelines, otherwise weak agree. 

black most likely nonshock violence (speculate, reporting on police violence). 
could be black content is over removed but hard to tel (n=1 compared to white 2). suppression as expected. nonwhite agree algo censored stronger than white. mixed and balck think against com guidelines, white and asian disagree. 

black and asian most likely post shock violence. censorship all on par. all agree alog censored, mixed and white most. all agree against com guidelines, white most. 

re mismatched, mostly agree reporting biggest cause except mixed who are more likely than any to agree to algo making one time mistake. 

RELIGION NOTES

comparing muslim to xtian and none (decent numbers, not clear whether athiest is norm, more common but uk context institutionally christian). 

muslim post least politics, and small count, but report same count of censorship as christian, so massively overrepresented. muslim not sure if algo censored, christain weak agree, no religio not sure (3.1). all disagree against com guidelines. 

similar likely some may find offensive. censorship on par. all agree algo censored, all agree against com guidelines. 

similar likely non erotic sex. muslim not sure algo censored, christ and none agree. disagree against com guidelines. 

no muslim post erotic, 10\% christian, 5\% none. all agree algo censored, muslim least. all agree against com guidelines, muslim least.
FOR DISCUSSION: (sometimes difference reflects lack of direct experience, sometimes not). 

christ post most covid. christ slightly more suppressed than none. christ not sure algo censored, muslim and none disagree. all disagree against com guidelines.

no big differences crit dom group. muslim not sure algo censored, christ and none agree, christ most. muslim not sure against com guidelines, christ agree, none disagree. 

similar likely SJ but only muslim report removal, overrepresented in suppression also. muslim not sure if algo censored, christ and none weak agree. all disagree against com guidelines, none most. 

muslim less likely post minority experience. all weakly agree algo censored. all weakly disagree against com guidelines. 

no muslims report posting hate speech, christ and none about 3-4\%. all agree algo censored, muslim least so, all agree against cmo guidelines, none most so, muslim least so. 
DISCUSSION: MINORITIES OFTEN LEAST LIKELY TO AGREE ALGO CENSORED, PERHAPS BECAUSE THEY ARE EXPOSED TO IT?

none group curses most. christians may be overrepresented in suppression compared to none. all weakly agree algo censored, all weakly disagree against com guidelines. 

muslim no self slurs, christian and none similar (5\%). on par censorship. christian and none weakly agree algo censored, muslim v weak (3.1). all weakly agree against com guidelines. 

nonshock violence and shock violence nothing interesting

nothing stands out re: mismatches. 
